The Complexity of Translationally-Invariant Low-Dimensional Spin Lattices in 3D

In this paper, we consider spin systems in three spatial dimensions, and prove that the local Hamiltonian problem for 3D lattices with face-centered cubic unit cells, 4-local translationally-invariant interactions between spin-3/2 particles and open boundary conditions is QMAEXP-complete. We go beyond a mere embedding of past hard 1D history state constructions, and utilize a classical Wang tiling problem as binary counter in order to translate one cube side length into a binary description for the verifier input. We further make use of a recently-developed computational model especially well-suited for history state constructions, and combine it with a specific circuit encoding shown to be universal for quantum computation. These novel techniques allow us to significantly lower the local spin dimension, surpassing the best translationally-invariant result to date by two orders of magnitude (in the number of degrees of freedom per coupling). This brings our models en par with the best non-translationally-invariant construction.

==> braket.tex <==
\RequirePackage{xparse}
\RequirePackage{amsmath}

% Bra-ket notation from physics.sty but without the other stuff
\DeclareDocumentCommand\bra{ s m t\ket s g }
{ % Bra
	\IfBooleanTF{#3}
	{ % Contraction
		\IfBooleanTF{#1}
		{ % Bra has a star: no resize
			\IfNoValueTF{#5}
			{\braket*{#2}{} \IfBooleanTF{#4}{*}{}}
			{\braket*{#2}{#5}}
		}
		{
			\IfBooleanTF{#4}
			{ % Ket has a star: no resize
				\IfNoValueTF{#5}
				{\braket{#2}{} *}
				{\braket*{#2}{#5}}
			}
			{\braket{#2}{\IfNoValueTF{#5}{}{#5}}} % Neither term is starred: auto sizing
		}
	}
	{ % No contraction
		\IfBooleanTF{#1}
		{\vphantom{#2}\left\langle\smash{#2}\right\rvert}
		{\left\langle{#2}\right\rvert}
		\IfBooleanTF{#4}{*}{}
		\IfNoValueTF{#5}{}{#5}
	}
}

\DeclareDocumentCommand\ket{ s m }
{ % Ket
	\IfBooleanTF{#1}
	{\vphantom{#2}\left\lvert\smash{#2}\right\rangle} % No resize
	{\left\lvert{#2}\right\rangle} % Auto sizing
}

\DeclareDocumentCommand\innerproduct{ s m g }
{ % Inner product
	\IfBooleanTF{#1}
	{ % No resize
		\IfNoValueTF{#3}
		{\vphantom{#2}\left\langle\smash{#2}\middle\vert\smash{#2}\right\rangle}
		{\vphantom{#2#3}\left\langle\smash{#2}\middle\vert\smash{#3}\right\rangle}
	}
	{ % Auto resize
		\IfNoValueTF{#3}
		{\left\langle{#2}\middle\vert{#2}\right\rangle}
		{\left\langle{#2}\middle\vert{#3}\right\rangle}
	}
}
\DeclareDocumentCommand\braket{}{\innerproduct} % Alternative for \innerproduct
	
\DeclareDocumentCommand\outerproduct{ s m g }
{ % Dyad
	\IfBooleanTF{#1}
	{ % No resize
		\IfNoValueTF{#3}
		{\vphantom{#2}\left\lvert\smash{#2}\middle\rangle\!\middle\langle\smash{#2}\right\rvert}
		{\vphantom{#2#3}\left\lvert\smash{#2}\middle\rangle\!\middle\langle\smash{#3}\right\rvert}
	}
	{ % Auto resize
		\IfNoValueTF{#3}
		{\left\lvert{#2}\middle\rangle\!\middle\langle{#2}\right\rvert}
		{\left\lvert{#2}\middle\rangle\!\middle\langle{#3}\right\rvert}
	}
}
\DeclareDocumentCommand\ketbra{}{\outerproduct} % Alternative for \outerproduct

